Counting and Finding Homomorphisms is Universal for Parameterized Complexity Theory

Counting homomorphisms from a graph $H$ into another graph $G$ is a fundamental problem of (parameterized) counting complexity theory. In this work, we study the case where \emph{both} graphs $H$ and $G$ stem from given classes of graphs: $H\in \mathcal{H}$ and $G\in \mathcal{G}$. By this, we combine the structurally restricted version of this problem, with the language-restricted version. Our main result is a construction based on Kneser graphs that associates every problem $\tt P$ in $\#\mathsf{W[1]}$ with two classes of graphs $\mathcal{H}$ and $\mathcal{G}$ such that the problem $\tt P$ is \emph{equivalent} to the problem $\#{\tt HOM}(\mathcal{H}\to \mathcal{G})$ of counting homomorphisms from a graph in $\mathcal{H}$ to a graph in $\mathcal{G}$. In view of Ladner's seminal work on the existence of $\mathsf{NP}$-intermediate problems [J.ACM'75] and its adaptations to the parameterized setting, a classification of the class $\#\mathsf{W[1]}$ in fixed-parameter tractable and $\#\mathsf{W[1]}$-complete cases is unlikely. Hence, obtaining a complete classification for the problem $\#{\tt HOM}(\mathcal{H}\to \mathcal{G})$ seems unlikely. Further, our proofs easily adapt to $\mathsf{W[1]}$. In search of complexity dichotomies, we hence turn to special graph classes. Those classes include line graphs, claw-free graphs, perfect graphs, and combinations thereof, and $F$-colorable graphs for fixed graphs $F$: If the class $\mathcal{G}$ is one of those classes and the class $\mathcal{H}$ is closed under taking minors, then we establish explicit criteria for the class $\mathcal{H}$ that partition the family of problems $\#{\tt HOM}(\mathcal{H}\to\mathcal{G})$ into polynomial-time solvable and $\#\mathsf{W[1]}$-hard cases. In particular, we can drop the condition of $\mathcal{H}$ being minor-closed for $F$-colorable graphs.

==> tikzlibraryconference.code.tex <==
%\documentclass{standalone}
%\usepackage{tikz}

\usepackage{ifthen}
\usetikzlibrary{calc,shapes,fit}

\tikzset{vertex/.style={circle, fill, inner sep=1pt, outer sep=1.3pt}}
\tikzset{svertex/.style={circle,draw=white, line width=1.2pt,fill=black, inner sep=1.8pt, outer sep=0pt}}
\tikzset{bag/.style={gray,minimum size=20pt,diamond,draw,rounded corners=4pt, inner sep=0pt, outer sep=-4pt, double=white, thick, fill=white}}
\tikzset{sbag/.style={gray,minimum size=15pt,diamond,draw,rounded corners=2pt, inner sep=0pt, outer sep=-4pt, double=white, thick, fill=white}}

\tikzset{hom/.style={black}}
\tikzset{shom/.style={white,double=black, thick}}

\def\ccol{red}
\def\ecol{blue}
\def\icol{red!50!blue}

\tikzset{dedge/.style={gray,thick, double=white, double distance=9pt}}
\tikzset{sdedge/.style={gray,thick, double=white, double distance=5pt}}

\tikzset{kneser style/.store in=\kneser@style,kneser style=10}

\tikzset{cross/.style={cross out, draw, minimum size=2*(#1-\pgflinewidth), inner sep=0pt, outer         sep=0pt}}
\tikzset{
    pics/encode/.style args={#1/#2/#3/#4}{
        % Encoding String -> Graph
        % #1 length of bitstring
        % #2 bitstring
        % #3 0/1: paths/both
        % #4 scale factor
        code = {
            \pgfmathsetmacro\mx{0}%
            \kneser@numtxt{\list}{#1}{0b#2}
            \foreach\x in {1,...,#1} {
                \node [vertex] (0\x) at (\x*#4, 0) {};
                \pgfmathsetmacro{\i}{int({\list}[\x-1])}
                \ifthenelse{#3=1}{
                    \node (0\x) at (\x*#4, -.5) {$\i$};
                }{}
                \ifthenelse{\i = 0}{}{
                    \global\let\mx=\x;
                    \foreach\j[count=\y from -1] in {0,...,\x}{
                        \node [vertex] (1\j) at (\x*#4, .35+ .45*\j) {};
                        \ifthenelse{\j=0}{}{
                            \draw[thick] (1\j) -- (1\y);
                        }
                    }
                }
            }
            \ifthenelse{#3=1}{
                \ifthenelse{\mx=0}{}{
                    \pgfmathsetmacro{\aspect}{.3/(.35+ .45*\mx+.3)};
                    \draw [decorate,decoration={brace,amplitude=5pt,aspect=\aspect}] (.35,-.15) -- (.   35,.35+ .45*\mx+.15);
                }
                \node (0) at (-.46, -.5) {$x$};
                \node (0) at (-.39, .15) {$\enc(x)$};
            }{}
        }
    }
}


\tikzset{
    pics/corner/.style args={#1/#2/#3}{
        code = {
            \pgfmathsetmacro{\bg}{int(div(\kneser@style,10))}
            \pgfmathsetmacro{\mode}{int(\kneser@style - \bg * 10)}
            \pgfmathsetmacro{\ax}{#1 < 0 ? .45 : -.45}
            \pgfmathsetmacro{\by}{#2 < 0 ? .45 : -.45}
            \pgfmathsetmacro{\nj}{#1==-#3?"1":(#1==#3?"k":"i")}
            \pgfmathsetmacro{\nl}{#2==#3?"1":(#2==-#3?"k":"j")}
            \fill[white] (\ax,0) -- (0,\by) -- (-\ax,0) -- (0,-\by) -- cycle;

            \ifthenelse{\mode=0}{
                \def\vs{svertex}
                \def\es{thick}
                \def\cl{\ccol}
            }{
                \def\cl{white}
                \def\vs{sbag}
                \def\es{sdedge}
            }


            \ifthenelse{\bg<3}{
                \node[\vs] at (\ax,0) (a) {};
                \node[\vs] at (0,\by) (b) {};
                \node[] at (0,-\by) {};
                \draw[white,double=\cl,\es] (a) to[\es] (b);
                \node[\vs,fill=\cl] at (\ax,0) {};
                \node[\vs,fill=\cl] at (0,\by) {};

                \ifthenelse{\mode=0}{
                    \begin{scope}[rotate=45]
                        \ifthenelse{#1=#2}{
                            \node[inner sep=0pt,outer sep=.2pt] at (\ax+\by/4.51,-\by/2) (a) {};
                            \node[inner sep=0pt,outer sep=.2pt] at (\by/4.51,\by-\by/2) (b) {};
                        }{
                            \node[inner sep=0pt,outer sep=.2pt] at (\ax-\ax/2,-\ax/4.51) (a) {};
                            \node[inner sep=0pt,outer sep=.2pt] at (-\ax/2,\by-\ax/4.51) (b) {};
                        }
                        \node[fit=(a)(b), rotate=-45,draw=white,double=\ccol!50, dashed,
                        rounded corners=2.8pt]{};
                    \end{scope}
                    \node[\ccol!50] at (-\ax/2,-\by/4) {\scriptsize $S(\nj,\nl)$};
                }{
                    \begin{scope}[rotate=45]
                        \ifthenelse{#1=#2}{
                            \node[inner sep=0pt,outer sep=7pt] at (\ax+\by/4.51,-\by/2) (a) {};
                            \node[inner sep=0pt,outer sep=7pt] at (\by/4.51,\by-\by/2) (b) {};
                        }{
                            \node[inner sep=0pt,outer sep=7pt] at (\ax-\ax/2,-\ax/4.51) (a) {};
                            \node[inner sep=0pt,outer sep=7pt] at (-\ax/2,\by-\ax/4.51) (b) {};
                        }
                        \node[fit=(a)(b), rotate=-45,draw=white,double=\ccol!50, dashed,
                        rounded corners=5pt]{};
                    \end{scope}
                    \node[\ccol!50] at (-\ax,-\by/1.2) {\scriptsize $S(c(\nj,\nl))$};

                }
            }{
                \node[\vs,outer sep=-1pt] at (\ax,1) (1) {};
                \node[\vs,outer sep=-1pt] at (\ax,.5) (a) {};
                \node[\vs,outer sep=-1pt] at (\ax,0) (c) {};
                \node[\vs,outer sep=-1pt] at (0,\by) (b) {};
                \node[\vs,outer sep=-1pt] at (0.5,\by) (3) {};
                \node[\vs,outer sep=-1pt] at (1,\by) (2) {};
                \node[] at (\ax*2.5,.5) (xa) {};
                \node[] at (\ax*2.5,0) (xc) {};
                \node[] at (0,\by*2.5) (xb) {};
                \node[] at (\ax*2.5,1) (x1) {};
                \node[] at (.5,\by*2.5) (x3) {};
                \node[] at (1,\by*2.5) (x2) {};
                \node[] at (0,-\by) {};
                \node[fit=(a)(c)(1), draw=gray,double=white,
                rounded corners=4pt]{};
                \node[fit=(b)(2)(3), draw=gray,double=white,
                rounded corners=4pt]{};
                \draw[white,double=gray] (a) to[\es] (xa);
                \draw[white,double=gray] (b) to[\es] (xb);
                \draw[white,double=gray] (c) to[\es] (xc);
                \draw[white,double=gray] (1) to[\es] (x1);
                \draw[white,double=gray] (2) to[\es] (x2);
                \draw[white,double=gray] (3) to[\es] (x3);
                \draw[white,double=\ccol] (a) to[\es] (b);
                \draw[white,double=\ccol] (c) to[\es] (b);
                \draw[white,double=\ccol] (c) to[\es] (a);
                \draw[white,double=\ccol!50] (1) to[\es] (2);
                \draw[white,double=\ccol!50] (3) to[\es] (2);
                \draw[white,double=\ccol!50] (3) to[\es] (1);
                \node[\vs,fill=\ccol] at (\ax,.5) {};
                \node[\vs,fill=\ccol] at (0,\by) {};
                \node[\vs,fill=\ccol] at (\ax,0) {};
                \node[\vs,fill=\ccol!50] at (\ax,1) {};
                \node[\vs,fill=\ccol!50] at (0.5,\by) {};
                \node[\vs,fill=\ccol!50] at (1,\by) {};
                \node at (\ax,1.35) {\scriptsize $c(\nj,\nl,\leftarrow)$};
                \node at (1.75,\by) {\scriptsize $c(\nj,\nl,\downarrow)$};
            }
        }
    }
}
\tikzset{
    pics/edge/.style args={#1/#2/#3}{
        code = {
            \pgfmathsetmacro{\bg}{int(div(\kneser@style,10))}
            \pgfmathsetmacro{\mode}{int(\kneser@style - \bg * 10)}

            \pgfmathsetmacro{\nj}{#1==-#3?"1":(#1==#3?"k":"i")}
            \pgfmathsetmacro{\nl}{#2==#3?"1":(#2==-#3?"k":"j")}
            \ifthenelse{\mode=0}{
                \def\vs{svertex}
                \def\es{thick}
                \def\cl{\ecol}
            }{
                \def\cl{white}
                \def\vs{sbag}
                \def\es{sdedge}
            }

            \pgfmathsetmacro{\ax}{#1 < 0 ? .45 : -.45}
            \pgfmathsetmacro{\by}{#2 < 0 ? .45 : -.45}
            \pgfmathsetmacro{\axx}{(#2 == -#3 || #2== #3) * (#1 < 0 ? .45 : -.45)}
            \pgfmathsetmacro{\byy}{(#1 == -#3 || #1== #3) * (#2 < 0 ? .45 : -.45)}
            \pgfmathsetmacro{\ay}{(#2 == -#3 || #2== #3) * (#2 < 0 ? -.45 : .45)}
            \pgfmathsetmacro{\bx}{(#1 == -#3 || #1== #3) * (#1 < 0 ? -.45 : .45)}

            \fill[white] (\ax,0) -- (0,\by) -- (-\ax,0) -- (0,-\by) -- cycle;

            \ifthenelse{\mode=0}{
                \pgfmathsetmacro{\xe}{(#1 == -#3 || #1== #3)}
                \ifthenelse{\bg<3}{
                    \ifthenelse{\xe=1}{
                        \draw[white,double=\ecol!50, dashed, rounded corners=2.2pt] (\ax*1.5,0)
                        -- (0,\by*1.5)
                        -- ($(0,\by*1.5)+0.35*(\bx, \ay)$)
                        -- ($(-\axx*1.5,-\byy*1.5)+0.35*(\bx, \ay)$)
                        -- (-\axx*1.5,-\byy*1.5)
                        -- cycle;
                    }{
                        \draw[white,double=\ecol!50, dashed, rounded corners=2.2pt] (\ax*1.5,0)
                        -- (0,\by*1.5)
                        -- (-\axx*1.5,-\byy*1.5)
                        -- ($(-\axx*1.5,-\byy*1.5)+0.35*(\bx, \ay)$)
                        -- ($(\ax*1.5,0)+0.35*(\bx, \ay)$)
                        -- cycle;
                    }
                    \node[\ecol!50] at (\bx*1.3,\ay*.9-\bx) {\scriptsize $S(\nj,\nl)$};
                }{
                }
            }{
                \pgfmathsetmacro{\xe}{(#1 == -#3 || #1== #3)}
                \ifthenelse{\bg<3}{
                    \ifthenelse{\xe=1}{
                        \draw[white,double=\ecol!50, dashed, rounded corners=4pt] (\ax*2.2,0)
                        -- (0,\by*2.2)
                        -- ($(0,\by*2.15)+(\bx, \ay)$)
                        -- ($(-\axx*2.15,-\byy*2.15)+(\bx, \ay)$)
                        -- (-\axx*2.2,-\byy*2.2)
                        -- cycle;
                    }{
                        \draw[white,double=\ecol!50, dashed, rounded corners=4pt] (\ax*2.2,0)
                        -- (0,\by*2.2)
                        -- (-\axx*2.2,-\byy*2.2)
                        -- ($(-\axx*2.15,-\byy*2.15)+(\bx, \ay)$)
                        -- ($(\ax*2.15,0)+(\bx, \ay)$)
                        -- cycle;
                    }
                    \node[\ecol!50] at (\bx*2.35,1.36*\ay+1.05*\bx) {\scriptsize $S(c(\nj,\nl))$};

                }{}
            }

            \ifthenelse{\bg<3}{
                \node[\vs] at (\ax,0) (a) {};
                \node[\vs] at (0,\by) (b) {};
                \node[\vs] at (-\axx,-\byy) (c) {};
                \node[] at (-\ax,0) {};
                \node[] at (0,-\by) {};
                \draw[white,double=\cl,\es] (a) to[\es] (b);
                \draw[white,double=\cl,\es] (a) to[\es] (c);
                \draw[white,double=\cl,\es] (b) to[\es] (c);
                \node[\vs,fill=\cl] at (\ax,0) {};
                \node[\vs,fill=\cl] at (0,\by) {};
                \node[\vs,fill=\cl] at (-\axx,-\byy) {};
            }{
                \node[\vs,outer sep=-1pt] at (\ax,1) (1) {};
                \node[\vs,outer sep=-1pt] at (\ax,.5) (a) {};
                \node[\vs,outer sep=-1pt] at (\ax,0) (c) {};
                \node[\vs,outer sep=-1pt] at (0,\by) (b) {};
                \node[\vs,outer sep=-1pt] at (0.5,\by) (3) {};
                \node[\vs,outer sep=-1pt] at (1,\by) (2) {};
                \node[\vs,outer sep=-1pt] at (-\ax+1,.75) (4) {};
                \node[\vs,outer sep=-1pt] at (-\ax+1,.25) (5) {};
                \node[] at (-\ax*2.5+1,.75) (x4) {};
                \node[] at (-\ax*2.5+1,.25) (x5) {};
                \node[] at (\ax*2.5,.5) (xa) {};
                \node[] at (\ax*2.5,0) (xc) {};
                \node[] at (0,\by*2.5) (xb) {};
                \node[] at (\ax*2.5,1) (x1) {};
                \node[] at (.5,\by*2.5) (x3) {};
                \node[] at (1,\by*2.5) (x2) {};
                \node[] at (0,-\by) {};
                \node[fit=(4)(5), draw=gray,double=white,
                rounded corners=4pt]{};
                \node[fit=(a)(c)(1), draw=gray,double=white,
                rounded corners=4pt]{};
                \node[fit=(b)(2)(3), draw=gray,double=white,
                rounded corners=4pt]{};
                \draw[white,double=gray] (4) to[\es] (x4);
                \draw[white,double=gray] (5) to[\es] (x5);
                \draw[white,double=gray] (a) to[\es] (xa);
                \draw[white,double=gray] (b) to[\es] (xb);
                \draw[white,double=gray] (c) to[\es] (xc);
                \draw[white,double=gray] (1) to[\es] (x1);
                \draw[white,double=gray] (2) to[\es] (x2);
                \draw[white,double=gray] (3) to[\es] (x3);
                \draw[white,double=\ecol] (a) to[\es] (b);
                \draw[white,double=\ecol] (c) to[\es] (b);
                \draw[white,double=\ecol] (c) to[\es] (a);
                \draw[white,double=\ecol] (a) to[\es] (3);
                \draw[white,double=\ecol] (c) to[\es] (3);
                \draw[white,double=\ecol] (b) to[\es] (3);
                \draw[white,double=\ecol!50] (2) to[\es] (1);
                \draw[white,double=\ecol!50] (4) to[\es] (1);
                \draw[white,double=\ecol!50] (5) to[\es] (1);
                \draw[white,double=\ecol!50] (5) to[\es] (4);
                \draw[white,double=\ecol!50] (2) to[\es] (4);
                \draw[white,double=\ecol!50] (2) to[\es] (5);
                \draw[\ecol] (a) to (b);
                \draw[\ecol!50] (1) to (5);
                \node[\vs,fill=\ecol] at (\ax,.5) {};
                \node[\vs,fill=\ecol] at (0,\by) {};
                \node[\vs,fill=\ecol] at (\ax,0) {};
                \node[\vs,fill=\ecol!50] at (\ax,1) {};
                \node[\vs,fill=\ecol] at (0.5,\by) {};
                \node[\vs,fill=\ecol!50] at (1,\by) {};
                \node[\vs,fill=\ecol!50] at (-\ax+1,.25) {};
                \node[\vs,fill=\ecol!50] at (-\ax+1,.75) {};
                \node at (\ax,1.35) {\scriptsize $c(\nj,\nl,\leftarrow)$};
                \node at (-\ax+1,1.15) {\scriptsize $c(\nj,\nl,\rightarrow)$};
                \node at (1.75,\by) {\scriptsize $c(\nj,\nl,\downarrow)$};
            }

        }
    }
}
\tikzset{
    pics/inner/.style args={#1/#2/#3}{
        code = {
            \pgfmathsetmacro{\bg}{int(div(\kneser@style,10))}
            \pgfmathsetmacro{\mode}{int(\kneser@style - \bg * 10)}

            \pgfmathsetmacro{\nj}{#1==-#3?"1":(#1==#3?"k":"i")}
            \pgfmathsetmacro{\nl}{#2==#3?"1":(#2==-#3?"k":"j")}
            \ifthenelse{\mode=0}{
                \def\vs{svertex}
                \def\cl{\icol}
                \def\es{thick}
                \pgfmathsetmacro{\ax}{.6}
                \pgfmathsetmacro{\by}{.6}
            }{
                \def\cl{white}
                \def\vs{sbag}
                \def\es{sdedge}
                \pgfmathsetmacro{\ax}{.8}
                \pgfmathsetmacro{\by}{.8}
            }

            \ifthenelse{\bg<3}{
                \fill[white] (\ax,0) -- (0,\by) -- (-\ax,0) -- (0,-\by) -- cycle;

                \node[\vs] at (\ax,0) (a) {};
                \node[\vs] at (0,\by) (b) {};
                \node[\vs] at (0,-\by) (c) {};
                \node[\vs] at (-\ax,0) (d) {};
                \node[diamond,minimum size=20pt] at (\ax,0) (a2) {};
                \node[diamond,minimum size=20pt] at (0,\by) (b2) {};
                \node[diamond,minimum size=20pt] at (0,-\by) (c2) {};
                \node[diamond,minimum size=20pt] at (-\ax,0) (d2) {};
                \node[\vs] at (\ax/2-\ax/4,-\by/2+\by/4) (e) {};
                \node[\vs] at (-\ax/2+\ax/4,\by/2-\by/4) (f) {};

                \node[] at (0,-\by) {};
                \draw[white,double=\cl,\es] (a) to[bend left] (c);
            }{}
            \ifthenelse{\mode=0}{
                \ifthenelse{\bg<3}{
                    \draw[white,double=\icol,thick] (c) -- (e) -- (a);
                    \draw[white,double=\icol,thick] (b) -- (f) -- (d);
                    \draw[white,double=\icol,thick] (e) -- (f);

                    \draw[white,double=\icol!50, dashed, rounded corners=2pt]
                    (\ax+.2,0)
                    to[bend right] (0,\by+.2)
                    to[bend right] (-\ax-.2,0)
                    to[bend right] (0,-\by-.2)
                    to[bend right] cycle;
                    \node[\icol!50] at (-\ax-.35,-\by) {\scriptsize $S(\nj,\nl)$};
                }{
                }
            }{
                \ifthenelse{\bg<3}{
                    \draw[white,double=\cl,\es] (c2) -- (e) -- (a2);
                    \draw[white,double=\cl,\es] (d2) -- (f) -- (b2);
                    \draw[white,double=\cl,\es] (e) -- (f);

                    \draw[white,double=\icol!50, dashed, rounded corners=5pt]
                    (\ax+.54,0)
                    to (0,\by+.54)
                    to (-\ax-.54,0)
                    to (0,-\by-.54)
                    -- cycle;
                    \node[\icol!50] at (-\ax-.3,-\by-.2) {\scriptsize $S(c(\nj,\nl))$};
                }{
                }

            }
            \ifthenelse{\bg<3}{
                \draw[white,double=\cl,\es] (b) to[bend right] (d);
                \node[\vs,fill=\cl] at (\ax,0) {};
                \node[\vs,fill=\cl] at (0,\by) {};
                \node[\vs,fill=\cl] at (0,-\by) {};
                \node[\vs,fill=\cl] at (-\ax,0) {};
                \node[\vs,fill=\cl] at (\ax/2-\ax/4,-\by/2+\by/4) {};
                \node[\vs,fill=\cl] at (-\ax/2+\ax/4,\by/2-\by/4) {};
            }{
                \node[\vs,outer sep=-1pt] at (\ax*2.5,-.5) (a) {};
                \node at (\ax*3.5,-.5) (xa) {};
                \node[\vs,outer sep=-1pt] at (\ax*2.5,0) (a2) {};
                \node at (\ax*3.5,0) (xa2) {};
                \node[\vs,outer sep=-1pt] at (\ax*2.5,.5) (a3) {};
                \node at (\ax*3.5,.5) (xa3) {};
                \node[\vs,outer sep=-1pt] at (-.25,\by*2.5) (b) {};
                \node at (-.25,\by*3.5) (xb) {};
                \node[\vs,outer sep=-1pt] at (.25,\by*2.5) (b2) {};
                \node at (.25,\by*3.5) (xb2) {};
                \node[\vs,outer sep=-1pt] at (-.25,-\by*2.5) (c) {};
                \node at (-.25,-\by*3.5) (xc) {};
                \node[\vs,outer sep=-1pt] at (.25,-\by*2.5) (c2) {};
                \node at (.25,-\by*3.5) (xc2) {};
                \node[\vs,outer sep=-1pt] at (-\ax*2.5,-.5) (d) {};
                \node at (-\ax*3.5,-.5) (xd) {};
                \node[\vs,outer sep=-1pt] at (-\ax*2.5,0) (d2) {};
                \node at (-\ax*3.5,0) (xd2) {};
                \node[\vs,outer sep=-1pt] at (-\ax*2.5,.5) (d3) {};
                \node at (-\ax*3.5,.5) (xd3) {};
                \node[svertex,outer sep=-1pt] at (\ax/2-.1,-\by/2) (ie) {};
                \node[svertex,outer sep=-1pt] at (-\ax/2-.2,\by/2) (if) {};
                \node[svertex,outer sep=-1pt] at (\ax/2+.2,-\by/2) (ie2) {};
                \node[svertex,outer sep=-1pt] at (-\ax/2+.1,\by/2) (if2) {};

                \node[fit=(a)(a2)(a3), draw=gray,double=white,
                rounded corners=4pt]{};
                \node[fit=(b)(b2), draw=gray,double=white,
                rounded corners=4pt]{};
                \node[fit=(c)(c2), draw=gray,double=white,
                rounded corners=4pt]{};
                \node[fit=(d)(d2)(d3), draw=gray,double=white,
                rounded corners=4pt]{};
                \node[fit=(ie)(ie2), draw=gray,double=white,
                rounded corners=4pt]{};
                \node[fit=(if)(if2), draw=gray,double=white,
                rounded corners=4pt]{};


                \draw[white,double=gray] (a) to[\es] (xa);
                \draw[white,double=gray] (a2) to[\es] (xa2);
                \draw[white,double=gray] (a3) to[\es] (xa3);
                \draw[white,double=gray] (b) to[\es] (xb);
                \draw[white,double=gray] (b2) to[\es] (xb2);
                \draw[white,double=gray] (c) to[\es] (xc);
                \draw[white,double=gray] (c2) to[\es] (xc2);
                \draw[white,double=gray] (d) to[\es] (xd);
                \draw[white,double=gray] (d2) to[\es] (xd2);
                \draw[white,double=gray] (d3) to[\es] (xd3);

                \draw[white,double=\icol,thick] (a2) -- (c) -- (ie2) -- (a);
                \draw[white,double=\icol,thick] (c) -- (a) -- (a2) -- (ie2);
                \draw[white,double=\icol,thick] (b) -- (d) -- (if2) -- (b);
                \draw[white, double=\icol, thick] (ie2) -- (if2);

                \draw[white,double=\icol!50,thick] (c2) -- (a3) -- (ie) -- (c2);
                \draw[white,double=\icol!50,thick] (d2) -- (b2) -- (if) -- (d3);
                \draw[white,double=\icol!50,thick] (b2) -- (d3) -- (d2) -- (if);
                \draw[white, double=\icol!50, thick] (ie) -- (if);

                \node[\vs,fill=\cl] at (\ax*2.5,-.5) {};
                \node[\vs,fill=\cl] at (\ax*2.5,0) {};
                \node[\vs,fill=\cl!50] at (\ax*2.5,.5) {};
                \node[\vs,fill=\cl] at (-.25,\by*2.5) {};
                \node[\vs,fill=\cl!50] at (.25,\by*2.5) {};
                \node[\vs,fill=\cl] at (-.25,-\by*2.5) {};
                \node[\vs,fill=\cl!50] at (.25,-\by*2.5) {};
                \node[\vs,fill=\cl] at (-\ax*2.5,-.5) {};
                \node[\vs,fill=\cl!50] at (-\ax*2.5,0) {};
                \node[\vs,fill=\cl!50] at (-\ax*2.5,.5) {};
                \node[\vs,fill=\cl] at (\ax/2+.2,-\by/2) {};
                \node[\vs,fill=\cl] at (-\ax/2+.1,\by/2) {};
                \node[\vs,fill=\cl!50] at (\ax/2-.1,-\by/2) {};
                \node[\vs,fill=\cl!50] at (-\ax/2-.2,\by/2) {};
                \node at (-\ax*2.5-.1,.9) {\scriptsize $c(\nj,\nl,\leftarrow)$};
                \node at (\ax*2.5,.9) {\scriptsize $c(\nj,\nl,\rightarrow)$};
                \node at (1,-\by*2.5) {\scriptsize $c(\nj,\nl,\downarrow)$};
                \node at (1,\by*2.5) {\scriptsize $c(\nj,\nl,\uparrow)$};
                \node at (\ax-.1,\by/2+.3) {\scriptsize $c(\nj,\nl,\nwarrow)$};
                \node at (-\ax/2-.2,-\by/2-.3) {\scriptsize $c(\nj,\nl,\searrow)$};
            }
        }
    }
}
\tikzset{
    pics/grid/.style args={#1}{
        code = {
            \pgfmathsetmacro{\bg}{int(div(\kneser@style,10))}
            \pgfmathsetmacro{\mode}{int(\kneser@style - \bg * 10)}

            \ifthenelse{\mode=0}{
                \pgfmathsetmacro{\dist}{\bg==2?.8:.6}
                \def\vs{vertex}
                \def\es{thick}
            }{
                \pgfmathsetmacro{\dist}{\bg==2?1.15:.9}
                \def\vs{bag}
                \def\es{dedge}
            }
            \pgfmathsetmacro{\n}{int(#1-1)}

            \foreach\i[count=\j from 1] in {-\n,...,\n}
            \foreach\k[count=\l from 1] in {-\n,...,\n}{
                \pgfmathsetmacro{\xedge}{\i==-\n || \i==\n}
                \pgfmathsetmacro{\yedge}{\k==-\n || \k==\n}
                \pgfmathsetmacro{\corner}{\xedge && \yedge}
                \pgfmathsetmacro{\edge}{\xedge || \yedge}

                \ifthenelse{\corner=1}{\def\tp{corner}\def\cl{\ccol}}
                {\ifthenelse{\edge=1}{\def\tp{edge}\def\cl{\ecol}}
                {\def\tp{inner}\def\cl{\icol}}}

                \pgfmathsetmacro{\bodd}{isodd(\j) && isodd(\l)}
                \ifthenelse{\bodd=1}{
                    \ifthenelse{\bg = 2}{
                        \node (\j\l) at (\dist*\i,\dist*\k) {};
                        \pic at (\dist*\i,\dist*\k) {\tp=\i/\k/\n};
                    }{
                        \node[\vs,\cl] (\j\l) at (\dist*\i,\dist*\k) {};
                        \pgfmathsetmacro{\nj}{\i==-\n?"1":(\i==\n?"k":"i")}
                        \pgfmathsetmacro{\nl}{\k==\n?"1":(\k==-\n?"k":"j")}
                        \ifthenelse{\mode=0}{
                            \node at (\dist*\i-.3,\dist*\k-.25) {\scriptsize$\nj, \nl$};
                        }{
                            \node at (\dist*\i-.65,\dist*\k-.45) {\scriptsize$c(\nj, \nl)$};
                        }
                    }
                    \ifthenelse{\j>1}{
                        \pgfmathsetmacro{\up}{int(\j-2)}
                        \draw[\es] (\up\l) -- (\j\l);
                    }{}
                    \ifthenelse{\l>1}{
                        \pgfmathsetmacro{\left}{int(\l-2)}
                        \draw[\es] (\j\left) -- (\j\l);
                    }{}
                }{}
            }


            % draw homomorphism and corrections
            \foreach\i[count=\j from 1] in {-\n,...,\n}
            \foreach\k[count=\l from 1] in {-\n,...,\n}{
                \pgfmathsetmacro{\xedge}{\i==-\n || \i==\n}
                \pgfmathsetmacro{\yedge}{\k==-\n || \k==\n}
                \pgfmathsetmacro{\corner}{\xedge && \yedge}
                \pgfmathsetmacro{\edge}{\xedge || \yedge}

                \ifthenelse{\corner=1}{\def\tp{corner}\def\cl{\ccol}}
                {\ifthenelse{\edge=1}{\def\tp{edge}\def\cl{\ecol}}
                {\def\tp{inner}\def\cl{\icol}}}

                \pgfmathsetmacro{\bodd}{isodd(\j) && isodd(\l)}
                \ifthenelse{\bodd=1}{
                    \ifthenelse{\bg=2}{
                        \node (\j\l) at (\dist*\i,\dist*\k) {};
                        \pic at (\dist*\i,\dist*\k) {\tp=\i/\k/\n};

                        \ifthenelse{\mode=0}{}{
                            \ifthenelse{\corner=1}{
                                \pgfmathsetmacro{\ax}{\i < 0 ? .45 : -.45}
                                \pgfmathsetmacro{\by}{\k < 0 ? .45 : -.45}
                                \node[vertex,\cl] at (\dist*\i+\ax+.07*rand,\dist*\k+.07*rand) (na\j\l) {};
                                \node[vertex,\cl] at (\dist*\i+.07*rand,\dist*\k+\by+.07*rand) (nb\j\l) {};
                                \draw[shom,double=\cl] (na\j\l) -- (nb\j\l);
                                \ifthenelse{\j>1}{
                                    \pgfmathsetmacro{\up}{int(\j-2)}
                                    \pgfmathsetmacro{\st}{"na\j\l"}
                                    \pgfmathsetmacro{\ed}{\i-2>=0?"nc\up\l":"na\up\l"}
                                    \draw[shom] (\st) -- (\ed);
                                }{}
                                \ifthenelse{\l>1}{
                                    \pgfmathsetmacro{\left}{int(\l-2)}
                                    \pgfmathsetmacro{\st}{"nb\j\l"}
                                    \pgfmathsetmacro{\ed}{\k-2>=0?"nc\j\left":"nb\j\left"}
                                    \draw[shom] (\st) -- (\ed);
                                }{}


                            }{
                                \ifthenelse{\edge=1}{
                                    \pgfmathsetmacro{\ax}{\i < 0 ? .45 : -.45}
                                    \pgfmathsetmacro{\by}{\k < 0 ? .45 : -.45}
                                    \pgfmathsetmacro{\axx}{(\k == -\n || \k== \n) * (\i < 0 ? .45 : -.45)}
                                    \pgfmathsetmacro{\byy}{(\i == -\n || \i== \n) * (\k < 0 ? .45 : -.45)}

                                    \node[vertex,\cl] at (\dist*\i+\ax+.07*rand,\dist*\k+.07*rand) (na\j\l) {};
                                    \node[vertex,\cl] at (\dist*\i+.07*rand,\dist*\k+\by+.07*rand) (nb\j\l) {};
                                    \node[vertex,\cl] at (\dist*\i+.07*rand-\axx,\dist*\k+.07*rand-\byy) (nc\j\l) {};

                                    \draw[shom,double=\cl] (na\j\l) -- (nb\j\l);
                                    \draw[shom,double=\cl] (na\j\l) -- (nc\j\l);
                                    \draw[shom,double=\cl] (nb\j\l) -- (nc\j\l);
                                    \ifthenelse{\j>1}{
                                        \pgfmathsetmacro{\up}{int(\j-2)}
                                        \ifthenelse{\xedge=1}{
                                            \draw[shom] (na\j\l) -- (na\up\l);
                                        }{
                                            \pgfmathsetmacro{\st}{\i>=0?"na\j\l":"nc\j\l"}
                                            \pgfmathsetmacro{\ed}{\i-2>=0?"nc\up\l":"na\up\l"}
                                            \draw[shom] (\st) -- (\ed);
                                        }
                                    }{}
                                    \ifthenelse{\l>1}{
                                        \pgfmathsetmacro{\left}{int(\l-2)}
                                        \ifthenelse{\yedge=1}{
                                            \draw[shom] (nb\j\l) -- (nb\j\left);
                                        }{
                                            \pgfmathsetmacro{\st}{\k>=0?"nb\j\l":"nc\j\l"}
                                            \pgfmathsetmacro{\ed}{\k-2>=0?"nc\j\left":"nb\j\left"}
                                            \draw[shom] (\st) -- (\ed);
                                        }
                                    }{}

                                }{
                                    \pgfmathsetmacro{\ax}{.8}
                                    \pgfmathsetmacro{\by}{.8}
                                    \node[vertex,\cl] at (\dist*\i+.05*rand+\ax,\dist*\k+.05*rand) (na\j\l) {};
                                    \node[vertex,\cl] at (\dist*\i+.05*rand,\dist*\k+.05*rand+\by) (nb\j\l) {};
                                    \node[vertex,\cl] at (\dist*\i+.05*rand,\dist*\k+.05*rand-\by) (nc\j\l) {};
                                    \node[vertex,\cl] at (\dist*\i+.05*rand-\ax,\dist*\k+.05*rand) (nd\j\l) {};
                                    \node[vertex,\cl] at (\dist*\i+\ax/2-\ax/4,\dist*\k-\by/2+\by/4) (ne\j\l) {};
                                    \node[vertex,\cl] at (\dist*\i-\ax/2+\ax/4,\dist*\k+\by/2-\by/4) (nf\j\l) {};

                                    \draw[shom,double=\cl] (na\j\l) to[bend left] (nc\j\l);
                                    \draw[shom,double=\cl] (na\j\l) -- (ne\j\l);
                                    \draw[shom,double=\cl] (ne\j\l) -- (nc\j\l);
                                    \draw[shom,double=\cl] (ne\j\l) -- (nf\j\l);
                                    \draw[shom,double=\cl] (nb\j\l) to[bend right] (nd\j\l);
                                    \draw[shom,double=\cl] (nb\j\l) -- (nf\j\l);
                                    \draw[shom,double=\cl] (nf\j\l) -- (nd\j\l);

                                    \pgfmathsetmacro{\up}{int(\j-2)}
                                    \pgfmathsetmacro{\left}{int(\l-2)}
                                    \draw[shom] (nb\j\left) -- (nc\j\l);
                                    \draw[shom] (na\up\l) -- (nd\j\l);


                                }
                            }
                        }
                    }{
                        \ifthenelse{\mode=0}{
                        }{
                            \node[bag] (\j\l) at (\dist*\i,\dist*\k) {};
                            \node[vertex,\cl] (n\j\l) at (\dist*\i+rand*.1,\dist*\k+rand*.1) {};
                            \ifthenelse{\j>1}{
                                \pgfmathsetmacro{\up}{int(\j-2)}
                                \draw[shom] (n\up\l) -- (n\j\l);
                            }{}
                            \ifthenelse{\l>1}{
                                \pgfmathsetmacro{\left}{int(\l-2)}
                                \draw[shom] (n\j\left) -- (n\j\l);
                            }{}
                        }
                    }
                }{}
            }
        }
    }
}


%\begin{document}
%\begin{tikzpicture}
%    \pic[style=1] {grid=4};
%    \pic at (-9,0) {grid=4};
%
%    \pic[style=20] at (-9, -9) {grid=4};
%    \pic[style=21] at (0, -9) {grid=4};
%\end{tikzpicture}
%\end{document}


==> tikzlibrarykneser.code.tex <==
\RequirePackage{ifthen}
\usetikzlibrary{calc}
\usetikzlibrary{shapes.geometric}

\makeatletter

\pgfmathdeclarefunction*{binom}{2}{%
    \begingroup
        \pgfmathcontinuelooptrue
        \c@pgf@counta=0
        \c@pgf@countb=1
        \c@pgf@countc=1
        \loop
        \ifpgfmathcontinueloop
            \ifnum\c@pgf@counta=#2\relax
                \pgfmathcontinueloopfalse
            \else
                \c@pgf@countd=#1
                \advance\c@pgf@countd by-\c@pgf@counta
                \multiply\c@pgf@countc by\c@pgf@countd
                \divide\c@pgf@countc by\c@pgf@countb
                \advance\c@pgf@counta by1\relax
                \advance\c@pgf@countb by1\relax
            \fi
        \repeat
        \pgfmathparse{int(\c@pgf@countc)}%
        \pgfmath@smuggleone\pgfmathresult
    \endgroup
}

\newcommand\kneser@intersect[4]{
    % Computes whether two given sets intersect, returns 1 if they intersect, 0 otherwise
    % #1 = variable to store the result
    % #2 = length
    % #3 = number 1 (base 10)
    % #4 = number 2 (base 10)
    \def\@res{0}

    \pgfmathsetmacro\@tmp{#3}%
    \pgfmathsetmacro\@tmpp{#4}%
    \foreach \@i in {1,...,#2}{%
        \pgfmathsetmacro\@ttmp{div(\@tmp,2)}%
        \pgfmathsetmacro\@ttmpp{div(\@tmpp,2)}%
        \pgfmathsetmacro{\@rr}{int(\@tmp - 2*\@ttmp)}%
        \pgfmathsetmacro{\@rrr}{int(\@tmpp - 2*\@ttmpp)}%
        \pgfmathsetmacro{\@rrrr}{int(\@rr * \@rrr)}%
        \ifthenelse{\@rrrr=1}{
            \global\def\@res{1}
            \breakforeach
        }{}
        \global\let\@tmp=\@ttmp%
        \global\let\@tmpp=\@ttmpp%
    }%

    \def#1{\@res}
}

\newcommand\kneser@numtxt[3]{%
    % Converts a bitstring into an array: 0b001 -> {0,0,1}
    % #1 = variable to store the list
    % #2 = length
    % #3 = number (base 10)
    \gdef\store@temp{\@gobble}%
    \pgfmathsetmacro\@tmp{#3}%
    \foreach \@i in {1,...,#2}{%
        \pgfmathsetmacro\@ttmp{div(\@tmp,2)}%
        \pgfmathparse{int(\@tmp - 2*\@ttmp)}%
        \xdef\store@temp{\store@temp,\pgfmathresult}%
        \global\let\@tmp=\@ttmp%
    }%
    \gdef\store@@temp{\@gobble}%
    \foreach \@i in {#2,...,1}{%
        \pgfmathparse{{\store@temp}[\@i-1]}%
        \xdef\store@@temp{\store@@temp,\pgfmathresult}%
    }%
    \let#1=\store@@temp%
}
\newcommand\kneser@numnext[3]{%
    % Generates next bitstring with same amount of 1's
    % #1 = variable to store the result
    % #2 = length
    % #3 = number (base 10)

    \gdef\store@temp{\@gobble}%
    \pgfmathsetmacro\@tmp{#3}%
    \foreach \@i in {1,...,#2}{%
        \pgfmathsetmacro\@ttmp{div(\@tmp,2)}%
        \pgfmathparse{int(\@tmp - 2*\@ttmp)}%
        \xdef\store@temp{\store@temp,\pgfmathresult}%
        \global\let\@tmp=\@ttmp%
    }%


    \def\@cnt{0}
    \def\@result{0}
    \def\@ca@r{1}
    \def\@done{0}
    \foreach \@i in {1,...,#2}{%
        \pgfmathsetmacro{\@cc}{{\store@temp}[\@i-1]}%
        \ifthenelse{\@done=1}{
            \ifthenelse{\@cc=1}{
                \pgfmathsetmacro{\@td@}{int(\@result+(\@cc*\@ca@r))}
                \global\let\@result=\@td@
            }{}
       }{
            \ifthenelse{\@cc=1}{
                \pgfmathsetmacro{\@t@mp}{int(\@cnt + 1)}
                \global\let\@cnt=\@t@mp%
            }{
                \ifthenelse{\@cnt>0}{
                    \global\def\@done{1}
                    \pgfmathsetmacro{\@t@}{int(\@result+\@ca@r)}
                    \global\let\@result=\@t@
                    \pgfmathsetmacro{\@tt@}{1}
                    \pgfmathsetmacro{\@ccnt@}{int(\@cnt-1)}
                    \ifthenelse{\@ccnt@>0}{
                    \foreach\@d in {1,...,\@ccnt@}{
                        \pgfmathsetmacro{\@td@}{int(\@result+\@tt@)}
                        \global\let\@result=\@td@
                        \pgfmathsetmacro{\@ttt@}{int(2*\@tt@)}
                        \global\let\@tt@=\@ttt@
                    }
                    }{}
                }{}
            }
        }
        \pgfmathsetmacro{\@ca@r@}{int(2*\@ca@r)}
        \global\let\@ca@r=\@ca@r@
    }

    \let#1=\@result
}
\newcommand\kneser@numidx[3]{%
    % Converts a bitstring into an array containing the indices being 1: 0b00110 -> {3,4}
    % #1 = variable to store the list
    % #2 = length
    % #3 = number (base 10)
    \gdef\store@temp{\@gobble}%
    \pgfmathsetmacro\@cnt{0}%
    \pgfmathsetmacro\@tmp{#3}%
    \foreach \@i in {1,...,#2}{%
        \pgfmathsetmacro\@ttmp{div(\@tmp,2)}%
        \pgfmathsetmacro\@r{int(\@tmp - 2*\@ttmp)}%
        \ifthenelse{\@r=1}{%
            \pgfmathsetmacro{\@s}{int(\@cnt+1)}%
            \global\let\@cnt=\@s%
            \pgfmathparse{int(#2-\@i+1)}%
            \xdef\store@temp{\store@temp,\pgfmathresult}%
        }{}%
        \global\let\@tmp=\@ttmp%
    }%
    \xdef\store@temp{\store@temp,}%
    \ifthenelse{\@cnt=0}{%
        \let#1=\empty%
    }{%
        \gdef\store@@temp{\@gobble}%
        \foreach \@i in {\@cnt,...,1}{%
            \pgfmathparse{{\store@temp}[\@i-1]}%
            \xdef\store@@temp{\store@@temp,\pgfmathresult}%
        }%
        \let#1=\store@@temp%
    }%
}

\tikzset{vertex fill color/.store in=\@vfc,vertex fill color=black}
\tikzset{vertex empty color/.store in=\@vec,vertex empty color=white}
\tikzset{kvertex/.style={circle, fill, inner sep=1.3pt, outer sep=1.8pt}}


\tikzset{kneser style/.store in=\kneser@style,kneser style=10}
    %   x0/x1/x2/x3 display mode: set/both/string/dot(without sets)
    %   0y/1y/2y background mode: empty/[fill color]/(unused)

\tikzset{edge fix/.store in=\rotfix,edge fix=0}
    % How to fix hidden edges:
    % 0: none
    % 1: use rotation by a small angle
    % 2: use bent edges

\tikzset{
    % Kneser set visualization
    % #1 length of bitstring
    % #2 bitstring
    pics/kneserset/.style args={#1/#2}{
        code = {
            \pgfmathsetmacro{\bg}{int(div(\kneser@style,10))}
            \pgfmathsetmacro{\mode}{int(\kneser@style - \bg * 10)}

            \ifthenelse{\mode<2}{
                \ifthenelse{#1=0}{}{
                    \kneser@numtxt{\arr}{#1}{0b#2}
                }
                \ifthenelse{\bg=0}{
                    \node[circle,minimum size=#1*2pt+16pt] () {};
                    \node[solid,circle,minimum size=#1*2pt+13pt,draw,thick]  {};
                }{
                   \ifthenelse{\mode>0}{
                        \kneser@numidx{\res}{#1}{0b#2}
                        \ifx\tikz@fillcolor\pgfutil@empty
                            \node[fill=white,inner sep=2pt,
                            rounded corners=5pt] (nn) at (0,-#1*1pt-14pt) {$\{\res\}$};
                        \else
                            \node[fill,inner sep=2pt,
                            rounded corners=5pt] (nn) at (0,-#1*1pt-14pt) {$\{\res\}$};
                        \fi
                    }{}
                    \ifx\tikz@fillcolor\pgfutil@empty
                        \node[circle,minimum size=#1*2pt+16pt,fill=white] () {};
                    \else
                        \node[fill,circle,minimum size=#1*2pt+16pt] () {};
                    \fi
                    \ifthenelse{\bg=1}{
                        \node[solid,circle,minimum size=#1*2pt+14pt,draw,thick]  {};
                    }{}
                    \node[circle,minimum size=#1*2pt+12pt,fill=white] {};
                }
                \ifthenelse{#1<3}{
                    \ifthenelse{#1<2}{
                        \ifthenelse{#1=0}{}{
                            \pgfmathsetmacro{\x}{{\arr}[0]}
                            \ifthenelse{\x=1}{
                                \node[solid,\@vfc,draw,fill=\@vfc,circle,inner sep=1.5pt] (1) at (0,0) {};
                            }{
                                \node[solid,\@vfc,draw,fill=\@vec,circle,inner sep=1.5pt] (1) at (0,0) {};
                            }
                        }
                    }{
                        \foreach \i in {1,...,#1} {
                            \pgfmathsetmacro{\x}{{\arr}[\i-1]}
                            \pgfmathsetmacro{\xx}{pow(-1,\i)*3}
                            \ifthenelse{\x=1}{
                                \node[solid,\@vfc,draw,fill=\@vfc,circle,inner sep=1.5pt](\i) at (\xx*1pt,0) {};
                            }{
                                \node[solid,\@vfc,draw,fill=\@vec,circle,inner sep=1.5pt](\i)at (\xx*1pt,0) {};
                            }
                        }
                    }
                }{
                    \node[regular polygon,regular polygon sides=#1,minimum size=#1*2pt,
                    inner sep=0pt] at (0,0) (poly#1) {};
                    \foreach \i in {1,...,#1} {
                        \pgfmathsetmacro{\x}{{\arr}[\i-1]}
                        \ifthenelse{\x=1}{
                            \node[solid,\@vfc,draw,fill=\@vfc,circle,inner sep=1.5pt]
                                (\i) at (poly#1.corner \i) {};
                        }{
                            \node[solid,\@vfc,draw,fill=\@vec,circle,inner sep=1.5pt] (\i)
                                at (poly#1.corner \i) {};
                        }
                    }
                }
            }{
                \kneser@numidx{\res}{#1}{0b#2}
                \ifx\tikz@fillcolor\pgfutil@empty
                    \node[fill=white,inner sep=1.5pt,rounded corners=5pt] () at (0,0) {$\{\res\}$};
                \else
                    \node[fill,inner sep=1.5pt,rounded corners=5pt] () at (0,0) {$\{\res\}$};
                \fi
            }
        }
    }
}

\def\ldraw(#1)--(#2);{
    \ifx\tikz@fillcolor\pgfutil@empty
        \draw[thick] (#1) -- (#2);
    \else
        \draw[thick,double=black,draw=\tikz@fillcolor] (#1) -- (#2);
    \fi
}
\def\bdraw(#1)--(#2);{
    \ifx\tikz@fillcolor\pgfutil@empty
        \draw[thick] (#1) to[bend left] (#2);
    \else
        \draw[thick,double=black,draw=\tikz@fillcolor] (#1) to[bend left] (#2);
    \fi
}



\def\lnode(#1)(#2);{
    \ifx\tikz@fillcolor\pgfutil@empty
        \node[kvertex,\@vfc,draw=white,line width=1pt] (#1) at (#2) {};
    \else
        \node[kvertex,\@vfc,draw=\tikz@fillcolor,line width=1pt] (#1) at (#2) {};
    \fi
}




\tikzset{
    % Draw Kneser Graph K(n,k)
    % #1 n
    % #2 k
    % Takes long if n > 7; dies if n > 9
    pics/kneser/.style args={#1/#2}{
        code = {
            \pgfmathsetmacro{\bg}{int(div(\kneser@style,10))}
            \pgfmathsetmacro{\mode}{int(\kneser@style - \bg * 10)}
            \pgfmathsetmacro{\done}{0}

            \pgfmathsetmacro{\diff}{int(#1-#2)}
            \pgfmathsetmacro{\db}{int(2*#2)}

            % K(n, 0)
            \ifthenelse{#2=0}{
                % 0 element subsets ~> boring
                \ifthenelse{\mode=3}{
                    \lnode(0)(0,0);
                }{
                    \pic (0) at (0,0) {kneserset=#1/0};
                }
                \pgfmathsetmacro{\done}{1}
            }{}

            % K(n, n)
            \ifthenelse{\done<1}{
                \ifthenelse{\diff=0}{
                    \pgfmathsetmacro{\all}{bin(int(pow(2,(#1+1))-1))}
                    \pgfmathsetmacro{\alll}{int(pow(2,(#1+1))-1)}
                    \ifthenelse{\mode=3}{
                        \lnode(\alll)(0,0);
                    }{
                        \pic at (0,0) (\alll) {kneserset=#1/\all};
                    }
                    \pgfmathsetmacro{\done}{1}
                }{}
            }{}

            % K(n, 1)
            \ifthenelse{\done<1}{
                \pgfmathsetmacro{\iscli}{#2==1&&#1>2}
                \ifthenelse{\iscli=1}{
                    % 1 element subsets ~> draw clique on n vertices

                    \ifthenelse{\mode=1}{
                        \node[regular polygon,regular polygon sides=#1,minimum size=#1*18pt]
                        (p#1) {};
                    }{
                        \node[regular polygon,regular polygon sides=#1,minimum size=#1*14pt]
                        (p#1) {};
                    }
                    \foreach \i in {#1,...,1} \foreach \j in {#1,...,1} {
                        \ifthenelse{\i=\j}{}{
                            \ldraw(p#1.corner \i)--(p#1.corner \j);
                        }
                    }
                    \foreach \i in {#1,...,1} \foreach \j in {#1,...,1} {
                        \ifthenelse{\i=\j}{}{
                            \draw[thick](p#1.corner \i)--(p#1.corner \j);
                        }
                    }

                    \def\tmp{1}
                    \foreach \i[count=\j from 1] in {#1,...,1} {
                        \edef\tp{\tmp}
                        \pgfmathsetmacro{\tmpint}{int(0b\tmp)}

                        \ifthenelse{\mode=3}{
                            \lnode(\tmpint)(p#1.corner \i);
                        }{
                            \pic[kneser style=1\mode] (\tmpint) at (p#1.corner \i) {kneserset=#1/\tmp};
                        }
                        \global\edef\tmp{\tp0}
                    }
                    \pgfmathsetmacro{\done}{1}
                }{}
            }{}

            % K(n, 2)
            \ifthenelse{\done<1}{
                \pgfmathsetmacro{\iscli}{#2==2&&#1>4}
                \ifthenelse{\iscli=1}{
                    \pgfmathsetmacro{\nmk}{int(#1 - #2)}
                    \pgfmathsetmacro{\nodd}{isodd(#1)}
                    \pgfmathsetmacro{\ncnt}{int(binom(#1,#2))}
                    \pgfmathsetmacro{\ecnt}{int(\ncnt*binom(\nmk,#2)/2)}

                    \pgfmathsetmacro{\nrem}{int(\ncnt)}
                    \pgfmathsetmacro{\nid}{int(0)}

                    \pgfmathsetmacro{\mxn}{int(pow(2,#1)-1)}

                    \pgfmathsetmacro{\rot}{int(isodd(#1) ? 0:-180/#1)}

                    \pgfmathsetmacro{\nly}{int(isodd(#1) ? div(\ncnt,#1) : 1 + div(\ncnt,#1))}
                    \pgfmathsetmacro{\lid}{int(1)}
                    \pgfmathsetmacro{\nexl}{int(1 + max(1,div(\nly,2)))}

                    \gdef\seen{\@gobble}
                    \gdef\poli{\@gobble}
                    \gdef\polc{\@gobble}
                    \ifthenelse{\nodd=1}{
                        \foreach\lid in {1,...,\nly}{
                            \pgfmathsetmacro{\ctm}{int(1 + pow(2,1+2*(\lid-1)))}
                            \foreach \j in {#1,...,1} {
                                \pgfmathsetmacro{\idx}{int(mod(\j + div(#1,2) - \lid, #1)+1)}
                                \pgfmathsetmacro{\curset}{bin(\ctm)}
                                \xdef\seen{\seen,\curset}
                                \xdef\poli{\poli,\lid}
                                \xdef\polc{\polc,\idx}

                                \pgfmathsetmacro{\ctmm}{int(2*\ctm > \mxn ? mod(2*\ctm + 1,\mxn+1) : 2*\ctm)}
                                \global\let\ctm=\ctmm
                            }
                        }

                        \foreach\ld in {1,...,\nexl}{
                            \pgfmathsetmacro{\doub}{int((#1<\nrem) && \ld>1)}
                            \ifthenelse{\doub=1}{
                                \pgfmathsetmacro{\tm}{int(\nrem - #1)}
                                \global\let\nrem=\tm
                                \pgfmathsetmacro{\rott}{int(-90/#1)}
                                %\pgfmathsetmacro{\rott}{int(0)}
                                \ifthenelse{\mode=1}{
                                    \node[regular polygon,regular polygon sides=#1,
                                    minimum size=#1*\ld*19pt-#1*3pt,
                                    rotate=\rot+\rott](p\lid){};
                                }{
                                    \node[regular polygon, regular polygon sides=#1,
                                    minimum size=#1*\ld*15pt-#1*3pt,
                                    rotate=\rot+\rott](p\lid){};
                                }
                                \pgfmathsetmacro{\tm}{int(\lid+1)}
                                \global\let\lid=\tm
                                \ifthenelse{\mode=1}{
                                    \node[regular polygon,regular polygon sides=#1,
                                    minimum size=#1*\ld*19pt-#1*3pt,
                                    rotate=\rot-\rott](p\lid){};
                                }{
                                    \node[regular polygon, regular polygon sides=#1,
                                    minimum size=#1*\ld*15pt-#1*3pt,
                                    rotate=\rot-\rott](p\lid){};
                                }
                                \pgfmathsetmacro{\tm}{int(\lid+1)}
                                \global\let\lid=\tm
                                \pgfmathsetmacro{\tm}{int(\nrem - #1)}
                                \global\let\nrem=\tm
                            }{
                                \ifthenelse{\rotfix=1}{
                                    \pgfmathsetmacro{\rott}{int(#1>5&&\lid==1?-#1/2:0)}
                                }{
                                    \pgfmathsetmacro{\rott}{int(0)}
                                }
                                \ifthenelse{\mode=1}{
                                    \node[regular polygon,regular polygon sides=#1,
                                    minimum size=#1*\ld*19pt-#1*3pt,
                                    rotate=\rott](p\lid){};
                                }{
                                    \node[regular polygon, regular polygon sides=#1,
                                    minimum size=#1*\ld*15pt-#1*3pt,
                                    rotate=\rott](p\lid){};
                                }
                                \pgfmathsetmacro{\tm}{int(\lid+1)}
                                \global\let\lid=\tm
                                \pgfmathsetmacro{\tm}{int(\nrem - #1)}
                                \global\let\nrem=\tm
                            }
                        }
                    }{
                        \pgfmathsetmacro{\rotsh}{iseven(#1/2)}
                        \foreach\lid in {1,...,\nly}{
                            \pgfmathsetmacro{\curn}{int((\lid==ceil(#1/4)&&not(\rotsh))
                            || (\lid==\nly && \rotsh)?#1/2:#1)}
                            \pgfmathsetmacro{\bnd}{int(int(\curn!=#1 ? 1 : \curn)}
                            \pgfmathsetmacro{\bend}{int(int(\curn!=#1 ? \curn :1)}
                            \pgfmathsetmacro{\ctm}{int(1 + pow(2,(\lid>ceil(#1/4) ? 0: 1)
                            +2*(\lid>ceil(#1/4)?\lid-div(#1,4):\lid-1)))}
                            \foreach \j in {\bnd,...,\bend} {
                                \ifthenelse{#1=6}{
                                    \pgfmathsetmacro{\idx}{int(mod(\j-2+\lid-(\lid==2), \curn)+1)}
                                }{}
                                \ifthenelse{#1=8}{
                                    \pgfmathsetmacro{\idx}{int(mod(\j-1*(\lid==1)+6*(\lid>1), \curn)+1)}
                                }{}
                                \ifthenelse{#1>8}{
                                    \pgfmathsetmacro{\idx}{int(mod(\j-1*(\lid==1)+6*(\lid>1), \curn)+1)}
                                }

                                \pgfmathsetmacro{\curset}{bin(\ctm)}
                                \xdef\seen{\seen,\curset}
                                \xdef\poli{\poli,\lid}
                                \xdef\polc{\polc,\idx}
                                \pgfmathsetmacro{\ctmm}{int(2*\ctm > \mxn ? mod(2*\ctm + 1,\mxn+1) : 2*\ctm)}
                                \global\let\ctm=\ctmm
                            }
                        }
                        \foreach\lid in {1,...,\nly}{
                            \pgfmathsetmacro{\level}{int(\lid>ceil(#1/4)?1+\lid-ceil(#1/4):\lid)}
                            \pgfmathsetmacro{\level}{#1==6&&\lid==3?1.8:\level}
                            \pgfmathsetmacro{\level}{#1==6&&\lid==1?1.07:\level}
                            \pgfmathsetmacro{\curn}{int((\lid==ceil(#1/4)&&not(\rotsh))
                            || (\lid==\nly && \rotsh)?#1/2:#1)}
                            \pgfmathsetmacro{\rott}{int((\lid>ceil(#1/4)&&\rotsh?180/#1:0)
                                + (not(\rotsh)&&\lid>1?-180/#1:0)
                            + (not(\rotsh)&&\curn!=#1?360/#1:0))}
                            \ifthenelse{\rotfix=1}{
                                \pgfmathsetmacro{\rott}{int(\lid==1?\rott-#1/2:\rott)}
                            }{}

                            \ifthenelse{\mode=1}{
                                \node[regular polygon,regular polygon sides=\curn,
                                minimum size=#1*\level*19pt-#1*3pt,
                                rotate=\rot+\rott](p\lid){};
                            }{
                                \node[regular polygon, regular polygon sides=\curn,
                                minimum size=#1*\level*15pt-#1*3pt,
                                rotate=\rot+\rott](p\lid){};
                            }
                        }
                    }
                    \ifthenelse{#1=6}{
                        \ifx\tikz@fillcolor\pgfutil@empty
                            \node[regular polygon,regular polygon sides=6, draw,
                            minimum size=#1*31.5pt,thick,rotate=0,rounded corners=10pt]{};
                        \else
                            \node[regular polygon,regular polygon sides=6,
                            double=black, draw=\tikz@fillcolor,
                            minimum size=#1*31.5pt,rotate=0,rounded corners=10pt]{};
                            \node[regular polygon,regular polygon sides=6, draw,
                            minimum size=#1*31.5pt,thick,rotate=0,rounded corners=10pt]{};
                        \fi
                    }{}

                    \gdef\prsx{\@gobble}
                    \gdef\prsy{\@gobble}
                    \foreach\i in {1,...,\ncnt}{
                        \pgfmathsetmacro{\curseta}{int({\seen}[\i-1])}
                        \pgfmathsetmacro{\cplia}{int({\poli}[\i-1])}
                        \pgfmathsetmacro{\cplca}{int({\polc}[\i-1])}
                        \foreach\j in {\i,...,\ncnt}{
                            \pgfmathsetmacro{\cursetb}{int({\seen}[\j-1])}
                            \pgfmathsetmacro{\cplib}{int({\poli}[\j-1])}
                            \pgfmathsetmacro{\cplcb}{int({\polc}[\j-1])}
                            \kneser@intersect{\inte}{#1}{0b\curseta}{0b\cursetb}
                            \pgfmathsetmacro{\outer}{\rotfix==2&&#1==6&&\cplia==2
                                                               &&\cplib==2}

                            \ifthenelse{\inte=0}{
                                \ifthenelse{\outer=0}{
                                \pgfmathsetmacro{\hb}{\rotfix==2&&#1==6&&\cplia+\cplib==3
                                                                &&\cplia!=\cplib&&(isodd(\cplca))}
                                    \ifthenelse{\hb=1}{
                                        \bdraw(p\cplia.corner \cplca)--(p\cplib.corner \cplcb);
                                    }{
                                        \ldraw(p\cplia.corner \cplca)--(p\cplib.corner \cplcb);
                                    }
                                }{}
                                \xdef\prsx{\prsx,\i}
                                \xdef\prsy{\prsy,\j}
                            }{}
                        }
                    }
                    \foreach\k in {1,...,\ecnt}{
                        \pgfmathsetmacro{\i}{int({\prsx}[\k-1])}
                        \pgfmathsetmacro{\j}{int({\prsy}[\k-1])}
                        \pgfmathsetmacro{\cplia}{int({\poli}[\i-1])}
                        \pgfmathsetmacro{\cplca}{int({\polc}[\i-1])}
                        \pgfmathsetmacro{\cplib}{int({\poli}[\j-1])}
                        \pgfmathsetmacro{\cplcb}{int({\polc}[\j-1])}
                        %\draw[thick](p\cplia.corner \cplca)--(p\cplib.corner \cplcb);

                        \pgfmathsetmacro{\outer}{\rotfix==2&&#1==6&&\cplia==2&&\cplib==2}
                        \pgfmathsetmacro{\hb}{\rotfix==2&&#1==6&&\cplia+\cplib==3
                        &&\cplia!=\cplib&&(isodd(\cplca))}
                        \ifthenelse{\outer=0}{
                        \ifthenelse{\hb=1}{
                            \draw[thick](p\cplia.corner \cplca) to[bend left]
                            (p\cplib.corner \cplcb);
                        }{
                            \draw[thick](p\cplia.corner \cplca)--(p\cplib.corner \cplcb);
                        }
                        }{}
                    }
                    \foreach\i in {1,...,\ncnt}{
                        \pgfmathsetmacro{\pli}{int({\poli}[\i-1])}
                        \pgfmathsetmacro{\plc}{int({\polc}[\i-1])}
                        \pgfmathsetmacro{\curset}{int({\seen}[\i-1])}
                        \pgfmathsetmacro{\curint}{int({\seen}[\i-1])}
                        \pgfmathsetmacro{\curint}{int(0b\curint)}

                        \ifthenelse{\mode=3}{
                            \lnode(\curint)(p\pli.corner \plc);
                        }{
                            \pic[kneser style=1\mode] (\curint) at (p\pli.corner \plc){kneserset=#1/\curset};
                        }
                    }
                    \pgfmathsetmacro{\done}{1}
                }{}
            }{}



            % K(2n, n)
            \ifthenelse{\done<1}{
                \ifthenelse{\db=#1}{
                    \pgfmathsetmacro{\all}{int(pow(2,(#1+1))-1)}
                    \pgfmathsetmacro{\tmo}{int(binom(#1,#2)/2-1)}
                    \pgfmathsetmacro{\tmr}{int(ceil(sqrt(\tmo*2)))}

                    \def\strt{0}
                    \foreach\d in {1,...,#2}{
                        \pgfmathsetmacro{\ttt}{int(2*\strt+1)}
                        \global\let\strt=\ttt
                    }

                    \ifthenelse{\tmr<5}{\pgfmathsetmacro\tmr{int(5)}}{}
                    \foreach\i[count=\j from 0] in {0,...,\tmo}{
                        \pgfmathsetmacro{\rem}{int(1+\tmo-(div(\j,\tmr)*\tmr))}
                        \ifthenelse{\rem>\tmr}{\pgfmathsetmacro\rem\tmr}{}

                        \pgfmathsetmacro{\nx}{int(-#1*2-12 + (-div(\tmo,\tmr)/2+div(\i,\tmr))*(#1*2+12+50+#1*2))}
                        \pgfmathsetmacro{\nxx}{int(#1*2+12 + (-div(\tmo,\tmr)/2+div(\i,\tmr))*(#1*2+12+50+#1*2))}

                        \ifthenelse{\mode=1}{\pgfmathsetmacro\dis{35}}
                        {\pgfmathsetmacro\dis{20}}

                        \pgfmathsetmacro{\ny}{(#1*2+\dis)*((\rem-1)/2 - mod(\i,\rem))}

                        \node (1\i) at (\nx*1pt,\ny*1pt) {};
                        \node (2\i) at (\nxx*1pt,\ny*1pt) {};
                        \ldraw(1\i)--(2\i);
                        \draw[thick](1\i)--(2\i);

                        \pgfmathsetmacro{\jj}{bin(int(\strt))}
                        \pgfmathsetmacro{\jd}{bin(int(\all-\strt))}
                        \pgfmathsetmacro{\jji}{(int(\strt))}
                        \pgfmathsetmacro{\jdi}{(int(\all-\strt))}

                        \ifthenelse{\mode=3}{
                            \lnode(\jji)(1\i);
                            \lnode(\jdi)(2\i);
                        }{
                            \pic[kneser style=1\mode] (\jji) at (1\i) {kneserset=#1/\jj};
                            \pic[kneser style=1\mode] (\jdi) at (2\i) {kneserset=#1/\jd};
                        }

                        \kneser@numnext{\tstrt}{#1}{\strt}
                        \global\let\strt=\tstrt
                    }
                    \pgfmathsetmacro{\done}{1}
                }{}
            }{}

            % K(n, n-1)
            \ifthenelse{\done<1}{
                \ifthenelse{\diff=1}{
                    \pgfmathsetmacro{\all}{int(pow(2,(#1+1))-1)}
                    \ifthenelse{\mode=1}{
                        \node[regular polygon,regular polygon sides=#1,minimum size=#1*18pt]
                        (p#1) {};
                    }{
                        \node[regular polygon,regular polygon sides=#1,minimum size=#1*14pt]
                        (p#1) {};
                    }
                    \def\tmp{1}
                    \foreach \i[count=\j from 1] in {#1,...,1} {
                        \edef\tp{\tmp}
                        \pgfmathsetmacro{\jd}{bin(int(\all-0b\tmp))}
                        \pgfmathsetmacro{\jdi}{int(\all-0b\tmp)}
                        \ifthenelse{\mode=3}{
                            \lnode(\jdi)(p#1.corner \i);
                            }{
                            \pic[kneser style=1\mode] (\jdi) at (p#1.corner \i) {kneserset=#1/\jd};
                        }
                        \global\edef\tmp{\tp0}
                    }
                    \pgfmathsetmacro{\done}{1}
                }{}
            }{}

            % K(n, k), k > n/2
            \ifthenelse{\done<1}{
                \ifthenelse{\db>#1}{
                    % No edges. Just draw the sets in a compact way
                    \pgfmathsetmacro{\tmo}{int(binom(#1,#2))}
                    \def\strt{0}
                    \foreach\d in {1,...,#2}{
                        \pgfmathsetmacro{\ttt}{int(2*\strt+1)}
                        \global\let\strt=\ttt
                    }
                    \pgfmathsetmacro{\tmr}{int(ceil(sqrt(\tmo)))}
                    \ifthenelse{\tmr<1}{\pgfmathsetmacro\tmr{int(1)}}{}

                    \foreach\i[count=\j from 0] in {1,...,\tmo}{
                        \pgfmathsetmacro{\rem}{int(\tmo-(div(\j,\tmr)*\tmr))}
                        \ifthenelse{\rem>\tmr}{\pgfmathsetmacro\rem\tmr}{}

                        \ifthenelse{\mode=1}{\pgfmathsetmacro\dis{35}}
                        {\pgfmathsetmacro\dis{20}}

                        \pgfmathsetmacro{\nx}{int((-div(\tmo,\tmr)/2+div(\j,\tmr))*(#1*2+\dis))}
                        \pgfmathsetmacro{\ny}{(#1*2+\dis)*((\rem-1)/2 - mod(\i,\rem))}

                        \pgfmathsetmacro{\cur}{bin(\strt)}

                        \ifthenelse{\mode=3}{
                            \lnode(\strt)(\nx*1pt,\ny*1pt);
                            }{
                            \pic (\strt) at (\nx*1pt,\ny*1pt) {kneserset=#1/\cur};
                        }

                        \kneser@numnext{\tstrt}{#1}{\strt}
                        \global\let\strt=\tstrt
                    }
                    \pgfmathsetmacro{\done}{1}
                }{}
            }{}

            % K(n, 3), n = 7
            \ifthenelse{\done<1}{
                % 5, 7, 9 1/3, 12, 15, 18 1/4 rings
                \pgfmathsetmacro{\sevthr}{#1==7 && #2==3}
                \gdef\seen{\@gobble}
                \gdef\poli{\@gobble}
                \gdef\polc{\@gobble}
                \pgfmathsetmacro{\nmk}{int(#1 - #2)}
                \pgfmathsetmacro{\ncnt}{int(binom(#1,#2))}
                \pgfmathsetmacro{\ecnt}{int(\ncnt*binom(\nmk,#2)/2)}
                \ifthenelse{\sevthr=1}{
                    \pgfmathsetmacro{\all}{int(pow(2,(#1))-1)}
                    \foreach\g in {1,...,3}{
                        \pgfmathsetmacro{\sca}{\g>1?\g*sqrt(sqrt(\g))/1.2:\g*1}
                        \ifthenelse{\mode=1}{
                            \node[regular polygon,regular polygon sides=#1,minimum size=#1*18pt*\g]
                            (p\g) {};
                        }{
                            \node[regular polygon,regular polygon sides=#1,
                            minimum size=#1*12pt*\sca] (p\g) {};
                        }
                    }
                    \ifthenelse{\mode=1}{
                        \node[regular polygon,regular polygon sides=2*#1,minimum size=#1*18pt*3.75]
                        (p4) {};
                    }{
                        \node[regular polygon,regular polygon sides=2*#1,
                        minimum size=#1*10.6pt*5] (p4) {};
                    }

                    % inner rings, vertices
                    \foreach\g in {1,...,3}{
                        % Yes, I am too lazy to generate the seeds automatically. . .
                        \pgfmathsetmacro{\tmp}{\g==1?7:(\g==2?int(0b1001010):int(0b110010))}
                        \foreach \i[count=\j from 1] in {#1,...,1} {
                            \pgfmathsetmacro{\idx}{int(mod(\i+5,#1)+1)}
                            \edef\tp{\tmp}
                            \pgfmathsetmacro{\tmpint}{\tmp}
                            \pgfmathsetmacro{\tmpbin}{bin(\tmp)}

                            \xdef\seen{\seen,\tmpbin}
                            \xdef\poli{\poli,\g}
                            \xdef\polc{\polc,\idx}
                            \pgfmathsetmacro{\tp}{2*\tmp>\all?int(mod(2*\tmp,\all)):int(2*\tmp)}
                            \global\edef\tmp{\tp}
                        }
                    }
                    % outer ring
                    \foreach \start[count=\s from 1] in {1010001,1000101}{
                        \pgfmathsetmacro{\tmp}{int(0b\start)}
                        \foreach \i[count=\j from 1] in {#1,...,1} {
                            \pgfmathsetmacro{\idx}{int(mod(2*\i+\s+5,2*#1)+1)}
                            \edef\tp{\tmp}
                            \pgfmathsetmacro{\tmpint}{\tmp}
                            \pgfmathsetmacro{\tmpbin}{bin(\tmp)}

                            \xdef\seen{\seen,\tmpbin}
                            \xdef\poli{\poli,4}
                            \xdef\polc{\polc,\idx}
                            \pgfmathsetmacro{\tp}{2*\tmp>\all?int(mod(2*\tmp,\all)):int(2*\tmp)}
                            \global\edef\tmp{\tp}
                        }
                    }
                    \gdef\prsx{\@gobble}
                    \gdef\prsy{\@gobble}
                    \foreach\i in {1,...,\ncnt}{
                        \pgfmathsetmacro{\curseta}{int({\seen}[\i-1])}
                        \pgfmathsetmacro{\cplia}{int({\poli}[\i-1])}
                        \pgfmathsetmacro{\cplca}{int({\polc}[\i-1])}
                        \foreach\j in {\i,...,\ncnt}{
                            \pgfmathsetmacro{\cursetb}{int({\seen}[\j-1])}
                            \pgfmathsetmacro{\cplib}{int({\poli}[\j-1])}
                            \pgfmathsetmacro{\cplcb}{int({\polc}[\j-1])}
                            \kneser@intersect{\inte}{#1}{0b\curseta}{0b\cursetb}
                            \ifthenelse{\inte=0}{
                                \pgfmathsetmacro{\hb}{\rotfix==2&&#1==6&&\cplia+\cplib==3
                                &&\cplia!=\cplib&&(isodd(\cplca))}
                                \ifthenelse{\hb=1}{
                                    \bdraw(p\cplia.corner \cplca)--(p\cplib.corner \cplcb);
                                }{
                                    \ldraw(p\cplia.corner \cplca)--(p\cplib.corner \cplcb);
                                }
                                \xdef\prsx{\prsx,\i}
                                \xdef\prsy{\prsy,\j}
                            }{}
                        }
                    }
                    \foreach\k in {1,...,\ecnt}{
                        \pgfmathsetmacro{\i}{int({\prsx}[\k-1])}
                        \pgfmathsetmacro{\j}{int({\prsy}[\k-1])}
                        \pgfmathsetmacro{\cplia}{int({\poli}[\i-1])}
                        \pgfmathsetmacro{\cplca}{int({\polc}[\i-1])}
                        \pgfmathsetmacro{\cplib}{int({\poli}[\j-1])}
                        \pgfmathsetmacro{\cplcb}{int({\polc}[\j-1])}

                        \pgfmathsetmacro{\hb}{\rotfix==2&&#1==6&&\cplia+\cplib==3
                        &&\cplia!=\cplib&&(isodd(\cplca))}
                        \ifthenelse{\hb=1}{
                            \draw[thick](p\cplia.corner \cplca) to[bend left]
                            (p\cplib.corner \cplcb);
                        }{
                            \draw[thick](p\cplia.corner \cplca)--(p\cplib.corner \cplcb);
                        }
                    }
                    \foreach\i in {1,...,\ncnt}{
                        \pgfmathsetmacro{\pli}{int({\poli}[\i-1])}
                        \pgfmathsetmacro{\plc}{int({\polc}[\i-1])}
                        \pgfmathsetmacro{\curset}{int({\seen}[\i-1])}
                        \pgfmathsetmacro{\curint}{int({\seen}[\i-1])}
                        \pgfmathsetmacro{\curint}{int(0b\curint)}

                        \ifthenelse{\mode=3}{
                            \lnode(\curint)(p\pli.corner \plc);
                        }{
                            \pic[kneser style=1\mode] (\curint) at (p\pli.corner \plc){kneserset=#1/\curset};
                        }
                    }

                    \pgfmathsetmacro{\done}{1}
                }{}
            }{}

            % K(n, k), general case
            \ifthenelse{\done<1}{
                \pgfmathsetmacro{\tmo}{int(binom(#1,#2))}
                \ifthenelse{\mode=1}{
                    \node[regular polygon,regular polygon sides=\tmo,minimum size=\tmo*20pt](o#1){};
                }{
                    \node[regular polygon,regular polygon sides=\tmo,minimum size=\tmo*10pt](o#1){};
                }
                \def\strt{0}
                \foreach\d in {1,...,#2}{
                    \pgfmathsetmacro{\ttt}{int(2*\strt+1)}
                    \global\let\strt=\ttt
                }
                \gdef\seen{\@gobble}
                \gdef\prsx{\@gobble}
                \gdef\prsy{\@gobble}
                \def\cnt{0}
                \foreach\i[count=\j from 0] in {1,...,\tmo}{
                    \ifthenelse{\j>0}{
                        \foreach\g in {1,...,\j}{
                            \pgfmathsetmacro{\cur}{int({\seen}[\g-1])}
                            \kneser@intersect{\inte}{#1}{\cur}{\strt}
                            \ifthenelse{\inte=0}{
                                \ldraw(o#1.corner \i)--(o#1.corner \g);
                                \xdef\prsx{\prsx,\i}
                                \xdef\prsy{\prsy,\g}
                                \pgfmathsetmacro{\gnr}{int(\cnt+1)}
                                \global\let\cnt=\gnr
                            }{}
                        }
                    }{}

                    \xdef\seen{\seen,\strt}
                    \kneser@numnext{\tstrt}{#1}{\strt}
                    \global\let\strt=\tstrt
                }
                \ifthenelse{\cnt>0}{
                    \foreach\i in {1,...,\cnt}{
                        \pgfmathsetmacro{\curx}{int({\prsx}[\i-1])}
                        \pgfmathsetmacro{\cury}{int({\prsy}[\i-1])}
                        \draw[thick](o#1.corner \curx)--(o#1.corner \cury);
                    }
                }{}
                \foreach\i[count=\j from 0] in {1,...,\tmo}{
                    \pgfmathsetmacro{\cur}{bin({\seen}[\j])}
                    \pgfmathsetmacro{\curint}{int({\seen}[\j])}

                    \ifthenelse{\mode=3}{
                        \lnode(\curint)(o#1.corner \i);
                    }{
                        \pic[kneser style=1\mode] (\curint) at (o#1.corner \i) {kneserset=#1/\cur};
                    }
                }
            }{}
        }
    }
}
\makeatother


